Bus Stop Spacings Statistics: Theory and Evidence

Transit agencies have been removing a large number of bus stops, but discussions around the bus stop spacings exhibit a lack of clarity and data for comparison. This paper proposes new terminology and concepts for statistical consideration of stop spacings, and introduces a python package and open-source database which uses General Transit Feed Specification data to derive real-world stop spacing distributions

==> tables/canada_stats.tex <==
\begin{tabular}{|l|c|}
    \hline
    \textbf{Attribute}                               & \textbf{Value} \\ \hline
    Segment Weighted Mean {[}m{]}                    & 394         \\ \hline
    Route Weighted Mean {[}m{]}                      & 373            \\ \hline
    Traversal Weighted Mean {[}m{]}                  & 357            \\ \hline
    No of Segments (Thousands)                       & 149            \\ \hline
    No of Routes                                     & 3742           \\ \hline
    No of Traversals (Million)                       & 7.3          \\ \hline
    \% Segments w/ spacing \textgreater threshold (3 km) & 1.53       \\ \hline
\end{tabular}%

==> tables/new_york.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Borough} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Segment \\ Weighted\\  Mean {[}m{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Route \\ Weighted \\ Mean {[}m{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traversal \\ Weighted\\  Mean {[}m{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\% Segments\\  w/ spacing \textgreater\\  threshold (3km)\end{tabular}} \\ \hline
Brooklyn                                                                         & 263          & 264          & 253          & 0.075          \\ \hline
Manhattan                                                                        & 271          & 262          & 261          & 0.126          \\ \hline
Staten Island                                                                    & 419          & 434          & 364          & 1.868          \\ \hline
Queens                                                                           & 309          & 300          & 266          & 0.163          \\ \hline
Bronx                                                                            & 344          & 335          & 333          & 0              \\ \hline
NYC Bus Company (Queens)                                                         & 377          & 391          & 335          & 0.992          \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}New York City MTA \\ (Combined)\end{tabular}} & \textbf{326} & \textbf{335} & \textbf{293} & \textbf{0.437} \\ \hline
\end{tabular}%

==> tables/top_cities.tex <==
\begin{tabular}{|p{8cm}|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Provider} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Urbanized \\ Area\end{tabular}} &
  \textbf{State} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Annual \\ Ridership \\ (Million)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Stop \\ Weighted \\ Mean {[}m{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Route \\ Weighted \\ Mean{[}m{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traversal \\ Weighted \\ Mean{[}m{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Segments \\ (1000s)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Routes\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Traversals \\ (1000s)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\% Segments \\ w/ spacing \textgreater  \\ threshold(3km)\end{tabular}} \\ \hline
MTA New York City Transit (NYCT)                            & New York        & NY & 692 & 312 & 320 & 284 & 14 & 245 & 1,561 & 0.32 \\ \hline
Los Angeles County Metropolitan   Transportation Authority    & Los Angeles     & CA & 267 & 405 & 401 & 388 & 13 & 112 & 805  & 0.54 \\ \hline
Chicago Transit Authority (CTA)                               & Chicago         & IL & 237 & 244 & 240 & 231 & 13 & 123 & 1,065 & 0.16 \\ \hline
Southeastern Pennsylvania Transportation   Authority (SEPTA)  & Philadelphia    & PA & 154 & 297 & 287 & 224 & 15 & 128 & 841  & 0.78 \\ \hline
New Jersey Transit (NJ Transit)                               & Newark          & NJ & 151 & 497 & 452 & 368 & 19 & 251 & 742  & 1.60 \\ \hline
Washington Metropolitan Area Transit   Authority (WMATA)      & Washington      & DC & 123 & 343 & 328 & 318 & 11 & 192 & 577  & 0.96 \\ \hline
San Francisco Municipal Transportation   Agency (SFMTA)       & San Francisco   & CA & 111 & 287 & 286 & 275 & 3  & 56  & 306  & 0.77 \\ \hline
King County Metro                                             & Seattle         & WA & 104 & 433 & 427 & 406 & 7  & 162 & 408  & 1.04 \\ \hline
Massachusetts Bay Transportation   Authority (MBTA)           & Boston          & MA & 100 & 317 & 308 & 301 & 8  & 159 & 371  & 0.65 \\ \hline
Regional Transportation District (RTD)                        & Denver          & CO & 70  & 435 & 438 & 399 & 8  & 105 & 274  & 0.66 \\ \hline
Regional Transportation Commission of   Southern Nevada (RTC) & Las Vegas       & NV & 64  & 494 & 493 & 490 & 4  & 39  & 169  & 1.12 \\ \hline
City and County of Honolulu (DTS)                             & Honolulu        & HI & 64  & 393 & 387 & 367 & 4  & 107 & 194  & 1.06 \\ \hline
Maryland Transit Administration                               & Baltimore       & MD & 64  & 434 & 404 & 352 & 5  & 65  & 286  & 1.00 \\ \hline
METRO Houston                                                 & Houston         & TX & 60  & 337 & 328 & 318 & 9  & 99  & 483  & 1.39 \\ \hline
TriMet, Portland Streetcar                                    & Portland        & OR & 56  & 367 & 365 & 343 & 7  & 83  & 269  & 0.20 \\ \hline
Port Authority of Allegheny County                            & Pittsburgh      & PA & 55  & 328 & 315 & 287 & 8  & 95  & 326  & 0.44 \\ \hline
Metro Transit                                                 & Minneapolis     & MN & 52  & 309 & 304 & 298 & 10 & 111 & 331  & 0.67 \\ \hline
Metropolitan Atlanta Rapid Transit   Authority (MARTA)        & Atlanta         & GA & 51  & 331 & 328 & 321 & 9  & 112 & 336  & 1.04 \\ \hline
Alameda-Contra Costa Transit District   (AC Transit)          & Oakland         & CA & 50  & 387 & 362 & 355 & 5  & 126 & 234  & 0.24 \\ \hline
San Diego Metropolitan Transit System   (MTS)                 & San Diego       & CA & 50  & 451 & 441 & 416 & 4  & 103 & 196  & 1.51 \\ \hline
Miami-Dade Transit                                            & Miami           & FL & 47  & 432 & 416 & 392 & 8  & 121 & 334  & 1.57 \\ \hline
VIA Metropolitan Transit (VIA)                                & San Antonio     & TX & 41  & 367 & 352 & 370 & 7  & 99  & 213  & 1.26 \\ \hline
Valley Metro (VM)                                             & Phoenix         & AZ & 41  & 460 & 454 & 436 & 8  & 112 & 361  & 0.33 \\ \hline
Orange County Transportation Authority   (OCTA)               & Orange County   & CA & 38  & 460 & 455 & 448 & 6  & 58  & 177  & 0.40 \\ \hline
Dallas Area Rapid Transit (DART)                              & Dallas          & TX & 37  & 334 & 327 & 327 & 7  & 95  & 324  & 0.97 \\ \hline
Milwaukee County Transit System (MCTS)                        & Milwaukee       & WI & 29  & 348 & 344 & 330 & 4  & 51  & 242  & 0.10 \\ \hline
Capital Metro                                                 & Austin          & TX & 28  & 544 & 514 & 508 & 3  & 72  & 134  & 1.40 \\ \hline
Santa Clara Valley Transportation   Authority (VTA)           & San Jose        & CA & 27  & 508 & 488 & 484 & 4  & 63  & 152  & 0.54 \\ \hline
Broward County Transit                                        & Fort Lauderdale & FL & 26  & 382 & 377 & 372 & 5  & 43  & 169  & 0.44 \\ \hline
Pace Bus                                                      & Chicago         & IL & 26  & 312 & 312 & 314 & 15 & 128 & 336  & 0.62 \\ \hline
\end{tabular}%
